RSSI-Based Location Classification Using a Particle Filter to Fuse Sensor Estimates

For Cyper-Physical Production Systems (CPPS), localization is becoming increasingly important as wireless and mobile devices are considered an integral part. While localizing targets in a wireless communication system based on the Received Signal Strength Indicators (RSSIs) is a usual solution, it is limited by sensor quality. We consider the scenario of a car moving in and out of a chamber and propose to use a particle filter for sensor fusion, allowing us to incorporate non-idealities in our model and achieve a high-quality position estimate. Then, we use Machine Learning (ML) to classify the vehicle position. Our results show that the location output of the particle filter is a better input to the classifiers than the raw RSSI data, and we achieve improved accuracy while simultaneously reducing the number of features that the ML has to consider. We also compare the performance of multiple ML algorithms and show that SVMs provide the overall best performance for the given task.

==> graphics/icassp_svm_acc_score_directional.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=2.3in,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.91)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={white!69.0196078431373!black},
xlabel={Nr. of samples \(\displaystyle N\)},
xmajorgrids,
xmin=-0.45, xmax=31.45,
xtick style={color=black},
xtick={-5,0,5,10,15,20,25,30,35},
xticklabels={\(\displaystyle {−5}\),\(\displaystyle {0}\),\(\displaystyle {5}\),\(\displaystyle {10}\),\(\displaystyle {15}\),\(\displaystyle {20}\),\(\displaystyle {25}\),\(\displaystyle {30}\),\(\displaystyle {35}\)},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy score},
ymajorgrids,
ymin=0.85, ymax=0.95,
ytick style={color=black},
ytick={0.84,0.86,0.88,0.9,0.92,0.94,0.96},
yticklabels={\(\displaystyle {0.84}\),\(\displaystyle {0.86}\),\(\displaystyle {0.88}\),\(\displaystyle {0.90}\),\(\displaystyle {0.92}\),\(\displaystyle {0.94}\),\(\displaystyle {0.96}\)}
]
\addplot [line width=1.5pt, color0]
table {%
1 0.819505200619734
2 0.844987760474525
3 0.858153057412328
4 0.864417971860346
5 0.869142109919343
6 0.871466764908303
7 0.872129795306776
8 0.87386514579921
9 0.87550411374906
10 0.876304413450766
11 0.875877195179526
12 0.876410004633392
13 0.875908831802624
14 0.87470164427026
15 0.87395902921036
16 0.872544616701855
17 0.871374468053852
18 0.870136568712539
19 0.868591579795641
20 0.867953355529599
21 0.866552714446422
22 0.865593937773436
23 0.864974676062926
24 0.864282833876385
25 0.863662182913802
26 0.863021621118434
27 0.862444627686305
28 0.862741972795611
29 0.863090666573965
30 0.863345092115611
};
\addlegendentry{SVM($\hat{\mathbf{p}})$}
\addplot [line width=1.5pt, color1, dashed]
table {%
1 0.847567364615697
2 0.870416951445269
3 0.87995563415667
4 0.884657612990787
5 0.887418775276423
6 0.890191162181229
7 0.89110945060586
8 0.894074526056237
9 0.896351198375277
10 0.898297686240067
11 0.900298363014143
12 0.901281523995181
13 0.902196509199946
14 0.903769436532454
15 0.904035113054221
16 0.904124211772586
17 0.905512549371183
18 0.905613839749361
19 0.905537317099281
20 0.904932041247547
21 0.904931744790166
22 0.903868283285825
23 0.903525828474514
24 0.902766852846828
25 0.901934371016498
26 0.9020198621743
27 0.902847000733224
28 0.903846692912327
29 0.904454652857072
30 0.904511770854157
};
\addlegendentry{SVM($\hat{\mathbf{p}}, \hat{\mathbf{\sigma}}^2$)}
\addplot [line width=1.5pt, color2, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 0.870204062647389
2 0.887603324541974
3 0.895487361965684
4 0.89920129371139
5 0.90278555520124
6 0.905127898752301
7 0.907198719175845
8 0.90921688288001
9 0.911443450031414
10 0.91189669975296
11 0.911284250604072
12 0.910983372255365
13 0.911331878170648
14 0.911832754584587
15 0.911188757506275
16 0.911372194423978
17 0.911273596453239
18 0.911828467951095
19 0.911457822268241
20 0.910436423269991
21 0.910295499480101
22 0.910257992831497
23 0.910336942780507
24 0.910611929942211
25 0.910505517813466
26 0.910405213332389
27 0.911311731060657
28 0.911846349150324
29 0.91231723071876
30 0.912644416147663
};
\addlegendentry{SVM($\hat{\mathbf{p}}, \hat{\mathbf{\sigma}}^2, \hat{\mathbf{v}}$)}
\addplot [line width=1.5pt, black, dotted]
table {%
1 0.856962070285938
2 0.883798131416837
3 0.894243307885733
4 0.897357135237103
5 0.901453897902958
6 0.903106783328677
7 0.90341209329402
8 0.904481764413422
9 0.903371386139672
10 0.903975056466082
11 0.904770157075666
12 0.904542774997174
13 0.90558415216089
14 0.904369617295422
15 0.904096210740917
16 0.904908959464933
17 0.905010986657179
18 0.903894260775222
19 0.903132433228389
20 0.90222828812438
21 0.902885597691576
22 0.902792016002403
23 0.901798039310414
24 0.901755028620024
25 0.902149773281444
26 0.902308706879979
27 0.902528335841975
28 0.902980149391655
29 0.902958244121191
30 0.90246537362302
};
\addlegendentry{SVM(RSSI Measurements)}
\addplot [line width=1.5pt, color0, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
12 0.876410004633392
};
\addplot [line width=1.5pt, color1, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
18 0.905613839749361
};
\addplot [line width=1.5pt, color2, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
30 0.912644416147663
};
\end{axis}

\end{tikzpicture}


==> graphics/icassp_svm_acc_score_omni.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=2.3in,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,0.91)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={white!69.0196078431373!black},
xlabel={Nr. of samples \(\displaystyle N\)},
xmajorgrids,
xmin=-0.45, xmax=31.45,
xtick style={color=black},
xtick={-5,0,5,10,15,20,25,30,35},
xticklabels={\(\displaystyle {−5}\),\(\displaystyle {0}\),\(\displaystyle {5}\),\(\displaystyle {10}\),\(\displaystyle {15}\),\(\displaystyle {20}\),\(\displaystyle {25}\),\(\displaystyle {30}\),\(\displaystyle {35}\)},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy score},
ymajorgrids,
ymin=0.85, ymax=0.95,
ytick style={color=black},
ytick={0.84,0.86,0.88,0.9,0.92,0.94,0.96},
yticklabels={\(\displaystyle {0.84}\),\(\displaystyle {0.86}\),\(\displaystyle {0.88}\),\(\displaystyle {0.90}\),\(\displaystyle {0.92}\),\(\displaystyle {0.94}\),\(\displaystyle {0.96}\)}
]
\addplot [line width=1.5pt, color0]
table {%
1 0.811123634452128
2 0.841032329984906
3 0.855582266114943
4 0.862938586450986
5 0.870532031319621
6 0.876435847854799
7 0.880707841840209
8 0.884020930780826
9 0.885868398157676
10 0.887011904041463
11 0.888718427119074
12 0.891674607744629
13 0.892538614968845
14 0.892377337575899
15 0.892730300343489
16 0.891678860379147
17 0.890900449566236
18 0.888925460104444
19 0.887959929258588
20 0.886706153221318
21 0.886312234986365
22 0.885460686437662
23 0.884534448325572
24 0.883811696575019
25 0.883132857268538
26 0.882983054755518
27 0.882127325424604
28 0.881109766571807
29 0.880866995779489
30 0.880111857113652
};
\addlegendentry{SVM($\hat{\mathbf{p}})$}
\addplot [line width=1.5pt, color1, dashed]
table {%
1 0.826846340345876
2 0.854599844367899
3 0.867717196057278
4 0.873165885406105
5 0.87838981211282
6 0.882169377659879
7 0.887075933562721
8 0.890693710280883
9 0.892870621338515
10 0.893925922838258
11 0.894792314622172
12 0.894631861612358
13 0.894542168413744
14 0.894110020293124
15 0.895261833605599
16 0.894916432630533
17 0.893464124328464
18 0.892502968818536
19 0.891498728244655
20 0.890877741429178
21 0.890928620450761
22 0.890448629944584
23 0.890595314838242
24 0.890479444447118
25 0.89053835995211
26 0.890024070973573
27 0.888676302075592
28 0.887367112315093
29 0.886599286383028
30 0.885083887288822
};
\addlegendentry{SVM($\hat{\mathbf{p}}, \hat{\mathbf{\sigma}}^2$)}
\addplot [line width=1.5pt, color2, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 0.859227916194169
2 0.875781449575168
3 0.886115197888281
4 0.895106333688922
5 0.899655634121603
6 0.901559417237485
7 0.904103066507886
8 0.9060217570258
9 0.907057261331125
10 0.906941272521047
11 0.907400072574708
12 0.90817992718627
13 0.907831373899547
14 0.906610145169347
15 0.90632078890966
16 0.905977048808262
17 0.905563474986635
18 0.905572974064063
19 0.905779652995628
20 0.906883578822133
21 0.906661643641746
22 0.906370981902631
23 0.905990677240489
24 0.905267654154098
25 0.904957926002789
26 0.904002663249134
27 0.903107950825144
28 0.901882339455898
29 0.901699450346358
30 0.900976490943276
};
\addlegendentry{SVM($\hat{\mathbf{p}}, \hat{\mathbf{\sigma}}^2, \hat{\mathbf{v}}$)}
\addplot [line width=1.5pt, black, dotted]
table {%
1 0.856962070285938
2 0.883798131416837
3 0.894243307885733
4 0.897357135237103
5 0.901453897902958
6 0.903106783328677
7 0.90341209329402
8 0.904481764413422
9 0.903371386139672
10 0.903975056466082
11 0.904770157075666
12 0.904542774997174
13 0.90558415216089
14 0.904369617295422
15 0.904096210740917
16 0.904908959464933
17 0.905010986657179
18 0.903894260775222
19 0.903132433228389
20 0.90222828812438
21 0.902885597691576
22 0.902792016002403
23 0.901798039310414
24 0.901755028620024
25 0.902149773281444
26 0.902308706879979
27 0.902528335841975
28 0.902980149391655
29 0.902958244121191
30 0.90246537362302
};
\addlegendentry{SVM(RSSI Measurements)}
\addplot [line width=1.5pt, color0, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
15 0.892730300343489
};
\addplot [line width=1.5pt, color1, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
15 0.895261833605599
};
\addplot [line width=1.5pt, color2, mark=asterisk, mark size=3, mark options={solid}, forget plot]
table {%
12 0.90817992718627
};
\end{axis}

\end{tikzpicture}

